The Challenges in Specifying and Explaining Synthesized Implementations of Reactive Systems

In formal synthesis of reactive systems an implementation of a system is automatically constructed from its formal specification. The great advantage of synthesis is that the resulting implementation is correct by construction; therefore there is no need for manual programming and tedious debugging tasks. Developers remain, nevertheless, hesitant to using automatic synthesis tools and still favor manually writing code. A common argument against synthesis is that the resulting implementation does not always give a clear picture on what decisions were made during the synthesis process. The outcome of synthesis tools is mostly unreadable and hinders the developer from understanding the functionality of the resulting implementation. Many attempts have been made in the last years to make the synthesis process more transparent to users. Either by structuring the outcome of synthesis tools or by providing additional automated support to help users with the specification process. In this paper we discuss the challenges in writing specifications for reactive systems and give a survey on what tools have been developed to guide users in specifying reactive systems and understanding the outcome of synthesis tools.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{B.~Finkbeiner and S.~Kleinberg: Third International Workshop\\ on Formal Reasoning about Causation, Responsibility,\\ and Explanations in Science and Technology (CREST 2018)\\
EPTCS 286, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.286.5}{10.4204/EPTCS.286.5}}
\pdfoutput=1

